Attacks in Adversarial Machine Learning: A Systematic Survey from the Life-cycle Perspective

Adversarial machine learning (AML) studies the adversarial phenomenon of machine learning, which may make inconsistent or unexpected predictions with humans. Some paradigms have been recently developed to explore this adversarial phenomenon occurring at different stages of a machine learning system, such as backdoor attack occurring at the pre-training, in-training and inference stage; weight attack occurring at the post-training, deployment and inference stage; adversarial attack occurring at the inference stage. However, although these adversarial paradigms share a common goal, their developments are almost independent, and there is still no big picture of AML. In this work, we aim to provide a unified perspective to the AML community to systematically review the overall progress of this field. We firstly provide a general definition about AML, and then propose a unified mathematical framework to covering existing attack paradigms. According to the proposed unified framework, we build a full taxonomy to systematically categorize and review existing representative methods for each paradigm. Besides, using this unified framework, it is easy to figure out the connections and differences among different attack paradigms, which may inspire future researchers to develop more advanced attack paradigms. Finally, to facilitate the viewing of the built taxonomy and the related literature in adversarial machine learning, we further provide a website, \ie, \url{http://adversarial-ml.com}, where the taxonomies and literature will be continuously updated.

==> tables/adversarial_category.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[t]
\centering
\renewcommand\arraystretch{1.4}
\caption{Summary of different categorizations of the adversarial examples.}
\label{tab: testing attacks}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l m{.31\textwidth} l m{.31\textwidth}}
\hline
\multicolumn{4}{c}{General formulation of inference-time adversarial examples:}                                                                                                                                                                                                                                                                                                                                                                                   \\
% \multicolumn{4}{c}{$\arg\min_{\x_{\varepsilon} \in \C_{\x}}~ \D_1(\x_0, \x_{\varepsilon}) + \lambda_1 \cL_1(f_{\w_0}(\x_{\varepsilon}), y_0) + \lambda_2 \cL_2(f_{\w_0}(\x_{\varepsilon}), y_{\varepsilon}) + \lambda_{r_1} \R_1(f_{\w_0}(\x_0), f_{\w_0}(\x_{\varepsilon})), ~ s.t. ~ \arg\max f_{\w_0}(\x_0) = y_0$}                                                  
\multicolumn{4}{c}{$\arg\min_{\x_{\varepsilon} \in \C_{\x}}~ \D_1(\x_0, \x_{\varepsilon}) + \lambda_3 \cL_3(f_{\w_0}(\x_{\varepsilon}), y_{\varepsilon}) + \lambda_{r_1} \R_1(f_{\w_0}(\x_0), f_{\w_0}(\x_{\varepsilon})), ~ s.t. ~ \arg\max f_{\w_0}(\x_0) = y_0$}                                                                                                                                                                                                                       \\ \hline\hline
\cellcolor[HTML]{DAE8FC}$\scriptscriptstyle\bigDiamond$ White-box                    & $f_{\w_0}(\cdot)$ is known to attacker                                                                                                                & \cellcolor[HTML]{DAE8FC}$\scriptscriptstyle\bigLozenge$ Black-box                    & $f_{\w_0}(\cdot)$ is unknown to attacker                                                                                                                                                                                                                \\ \hline
\multicolumn{4}{c}{Attacks with different perturbation types}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \hline
\cellcolor[HTML]{FFF2CC}$\scriptscriptstyle\bigDiamond$ Digital                      & The whole process of generating $\x_{\varepsilon}$ is conducted in the digital space                                                                  & \cellcolor[HTML]{FFF2CC}$\scriptscriptstyle\bigLozenge$ Physical                     & $\x_{\varepsilon}$ is transformed between the digital and physical space, \ie, $\x_{\varepsilon} \leftarrow D2P(\x_{\varepsilon})$, with $D2P(\cdot)$ indicating the transformation from digital to physical, then back to digital space \\
\cellcolor[HTML]{FFF2CC}$\scriptscriptstyle\bigDiamond$ Optimization-based           & $\x_{\varepsilon}$ is obtained \{\it w.r.t.\} each $\x_0$ by solving the above optimization problem                                    & \cellcolor[HTML]{FFF2CC}$\scriptscriptstyle\bigLozenge$ Learning-based               & Generating $\x_{\varepsilon}$ directly through a parametric model, \ie, $\x_{\varepsilon} = g_{\btheta}(\x_0)$                                                                                                                           \\
\cellcolor[HTML]{FFF2CC}$\scriptscriptstyle\bigDiamond$ Sample-agnostic perturbation & $\x_{\varepsilon} - \x_0$ is independent with $\x_0$                                                                                                  & \cellcolor[HTML]{FFF2CC}$\scriptscriptstyle\bigLozenge$ Sample-specific perturbation & $\x_{\varepsilon} - \x_0$ is dependent on $\x_0$                                                                                                                                                                                                        \\
\cellcolor[HTML]{FFF2CC}$\scriptscriptstyle\bigDiamond$ Additive perturbation        & The poisoned sample $\x_{\varepsilon}$ looks inconsistent with its label $y_{\varepsilon}$, from human's perspective                                  & \cellcolor[HTML]{FFF2CC}$\scriptscriptstyle\bigLozenge$ Non-additive perturbation    & $\x_{\varepsilon} = h(\x_0)$, with $h(\cdot)$ being a global transformation, \eg, spatial transformation or style transfer                                                                                                               \\
\cellcolor[HTML]{FFF2CC}$\scriptscriptstyle\bigDiamond$ Dense perturbation           & $\|\x_{\varepsilon} -\x_0 \|_0 = |\x_0|$, with $|\x_0|$ being the dimension of $\x_0$, \ie, all entries/pixels of $\x_0$ are perturbed & \cellcolor[HTML]{FFF2CC}$\scriptscriptstyle\bigLozenge$ Sparse perturbation          & $\|\x_{\varepsilon} -\x_0 \|_0 < |\x_0|$, \ie, only partial entries/pixels of $\x_0$ are perturbed                                                                                                                          \\ \hline\hline
\multicolumn{4}{c}{Attacks with different output types}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
\cellcolor[HTML]{D5E8D4}$\scriptscriptstyle\bigDiamond$ Untargeted                   & $y_{\varepsilon} = y_0$, and $\cL_3$ could be specified as the negative cross entropy loss or negative hinge loss        & \cellcolor[HTML]{D5E8D4}$\scriptscriptstyle\bigLozenge$ Targeted                     & $y_{\varepsilon} \neq y_0$, $\cL_2$ could be specified as the cross entropy loss or hinge loss                                                       \\
\cellcolor[HTML]{D5E8D4}$\scriptscriptstyle\bigDiamond$ Factorized output            & $f_{\w_0}(\cdot)$ is factorized, \eg, the CNN model for image classification or segmentation                                           & \cellcolor[HTML]{D5E8D4}$\scriptscriptstyle\bigLozenge$ Structured output            & $f_{\w_0}(\cdot)$ is structured, \eg, the RNN model for image-captioning or language translation                                                                                                                                         \\ \hline
\end{tabular}%
}
\end{table*}

==> tables/adversarial_papers.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[!h]
\caption{Categorization of existing adversarial attack methods. For any classification criterion ``A/B'', \Circle ~ denotes the former ``A'', \CIRCLE ~ denotes the latter ``B''.}
\label{tab:adversarial papers}
\resizebox{\textwidth}{!}{%
\begin{tabular}
{
m{0.09\textwidth}
m{0.09\textwidth}
|
m{0.07\textwidth}<{\centering}
m{0.07\textwidth}<{\centering}
m{0.07\textwidth}<{\centering}
m{0.07\textwidth}<{\centering}
m{0.07\textwidth}<{\centering}
m{0.07\textwidth}<{\centering}
m{0.07\textwidth}<{\centering}
|
m{0.07\textwidth}<{\centering}
m{0.07\textwidth}<{\centering}
}
\hline
                                                   &                           & \multicolumn{7}{c|}{White-box attack}   & Black-box attack & Transfer-based attack \\
Method &
  Venue &
  \cellcolor[HTML]{FFF2CC}Digtial / Physical &
  \cellcolor[HTML]{FFF2CC}Optimization / Learning-based &
  \cellcolor[HTML]{FFF2CC}Sample-agnostic / specific &
  \cellcolor[HTML]{FFF2CC}Additive / Non-additive &
  \cellcolor[HTML]{FFF2CC}Dense / Sparse &
  \cellcolor[HTML]{D5E8D4}Untargeted / Targeted &
  \cellcolor[HTML]{D5E8D4}Factorized / Structured &
  \cellcolor[HTML]{E1D5E7}Decison / Score-based &
  \cellcolor[HTML]{E1D5E7}Example / Model-level \\ \hline
Sharif \etal \cite{sharif2016accessorize}          & CCS 2016                  & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Kurakin \etal \cite{kurakin2018adversarial}        & ICLR 2017                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
UAP  \cite{moosavi2017universal}                   & CVPR 2017                 & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle &                  &                       \\
JSMA \cite{papernot2016limitations}                & EuroS\&P 2016             & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
Mopuri \etal \cite{mopuri2017fast}                 & BMVA 2017                 & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Carlini \etal \cite{carlini2017towards}            & IEEE S\&P 2017            & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
LocSearchAdv \cite{NarodytskaK16}                  & CVPR 2017                 & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
GD-UAP \cite{gd-uap-tpami-2018}                    & IEEE TPAMI 2018           & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Carlini \etal \cite{carlini2018audio}              & IEEE SPW 2018             & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \CIRCLE &                  &                       \\
ShapeShifter \cite{chen2018shapeshifter}           & ECML-PKDD 2018            & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
RP2 \cite{eykholt2018robust}                       & CVPR 2018                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Xu \etal \cite{xu2018fooling}                      & CVPR 2018                 & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \CIRCLE &                  &                       \\
Manifool \cite{kanbak2018geometric}                & CVPR 2018                 & \Circle & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle &                  &                       \\
Shi \etal \cite{shi2018learning}                   & COLING 2018               & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \CIRCLE &                  &                       \\
AC-GAN \cite{song2018constructing}                 & NeurIPS 2018              & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
advGAN \cite{xiao2018generating}                   & IJCAI 2018                & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
stAdv \cite{xiao2018spatially}                     & ICLR 2018                 & \Circle & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle &                  &                       \\
Athalye \cite{athalye2018synthesizing}             & ICML 2018                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
LaVAN \cite{karmon2018lavan}                       & ICML 2018                 & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
CGAN-Adv \cite{yu2018generating}                   & ICPR 2018                 & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Zhao \etal \cite{zhao2018admm}                     & MM 2018                   & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
Chen \etal \cite{chen2018attacking}                & ACL 2018                  & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \CIRCLE &                  &                       \\
Jan \etal \cite{jan2019connecting}                 & AAAI 2019                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Wei \etal \cite{WeiZYS19}                          & AAAI 2019                 & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
PS-GAN \cite{liu2019perceptual}                    & AAAI 2019                 & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
ERCG \cite{zhao2019seeing}                         & CCS 2019                  & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Qin \etal \cite{qin2019imperceptible}              & ICML 2019                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Engstrom \etal \cite{engstrom2019exploring}        & ICML 2019                 & \Circle & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle &                  &                       \\
Wong \etal \cite{wong2019wasserstein}              & ICML 2019                 & \Circle & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle &                  &                       \\
ReColorAdv \cite{laidlaw2019functional}            & NeurIPS 2019              & \Circle & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle &                  &                       \\
AT-GAN \cite{wang2019gan}                          & arXiv 2019                & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Yakura \etal \cite{yakura2018robust}               & IJCAI 2019                & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
AdvFaces  \cite{deb2019advfaces}                   & IJCB 2019                 & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
AGNs \cite{sharif2019general}                      & TOPS 2019                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
SparseFool \cite{ModasMF19}                        & CVPR 2019                 & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
Xu \etal \cite{xu2019exact}                        & CVPR 2019                 & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \CIRCLE &                  &                       \\
AdvPattern \cite{wang2019advpattern}               & ICCV 2019                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
CornerSearch \cite{croce2019sparse}                & ICCV 2019                 & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
PD-UA \cite{liu2019universal}                      & ICCV 2019                 & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Schott \etal \cite{SchottRBB19}                    & ICLR 2019                 & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
Xu \etal \cite{xu2018structured}                   & ICLR 2019                 & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
Su \etal \cite{su2019one}                          & IEEE TEC 2019             & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
CD-UAP \cite{cd-uap-aaai-2020}                     & AAAI 2020                 & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Xu \etal \cite{tshirt}                             & ECCV 2020                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Wu \etal \cite{wu2020making}                       & ECCV 2020                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
SAPF \cite{my-eccv-sparse}                         & ECCV 2020                 & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
UPC  \cite{huang2020universal}                     & CVPR 2020                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
AdvCam \cite{duan2020adversarial}                  & CVPR 2020                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
LG-GAN \cite{zhou2020lg}                           & CVPR 2020                 & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Xu \etal \cite{xu2020machines}                     & CVPR 2020                 & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \CIRCLE &                  &                       \\
PhysGAN \cite{kong2020physgan}                     & CVPR 2020                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Li \etal \cite{li2020towards}                      & CVPR 2020                 & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \CIRCLE & \Circle &                  &                       \\
GreedyFool \cite{LiuZGAL20}                        & NeurIPS 2020              & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
Xu \etal \cite{xu2020learning}                     & MM 2020                   & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \CIRCLE &                  &                       \\
MAG-GAN \cite{chen2020mag}                         & Information Sciences 2020 & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
GUAP \cite{zhang2020generalizing}                  & ICDM 2020                 & \Circle & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle &                  &                       \\
Wong \etal \cite{wong2020learning}                 & ICLR 2021                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
AdvHat \cite{komkov2021advhat}                     & ICPR 2021                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Sayles \etal \cite{sayles2021invisible}            & CVPR 2021                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
TTP \cite{naseer2021generating}                    & ICCV 2021                 & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \CIRCLE & \Circle &                  &                       \\
CMML  \cite{feng2021meta}                          & ICCV 2021                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Zhao \etal \cite{zhao2021success}                  & NeurIPS 2021              & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \CIRCLE & \Circle &                  &                       \\
SLAP \cite{lovisotto2021slap}                      & USENIX Security 2021      & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
AP-GAN \cite{zhao2020ap}                           & Geoinformatica 2022       & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\ \hline\hline
Brendel \etal \cite{brendel2018decision}           & ICLR 2018                 &     &     &     &     &     &     &     & \Circle              &                       \\
Ilyas \etal \cite{ilyas2018black}                  & ICML 2018                 &     &     &     &     &     &     &     & \Circle              &                       \\
NES \cite{ilyas2018black}                          & ICML 2018                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
GAP \cite{gap-2018}                                & CVPR 2018                 &     &     &     &     &     &     &     &                  & \Circle                   \\
MI-FGSM \cite{dong2018boosting}                    & CVPR 2018                 &     &     &     &     &     &     &     &                  & \CIRCLE                   \\
OPT \cite{cheng2019query}                          & ICLR 2019                 &     &     &     &     &     &     &     & \Circle              &                       \\
Sign-OPT \cite{cheng2019improving}                 & NeurIPS 2019              &     &     &     &     &     &     &     & \Circle              &                       \\
Subspace attack \cite{guo2019subspace}             & NeurIPS 2019              &     &     &     &     &     &     &     & \CIRCLE              &                       \\
Naseer \etal \cite{naseer2019cross}                & NeurIPS 2019              &     &     &     &     &     &     &     & \Circle              & \Circle                   \\
qFool \cite{liu2019geometry}                       & ICCV 2019                 &     &     &     &     &     &     &     & \Circle              &                       \\
ILAP \cite{huang2019enhancing}                     & ICCV 2019                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
SimBA \cite{guo2019simple}                         & ICML 2019                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
ECO \cite{moon2019parsimonious}                    & ICML 2019                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
NAttack  \cite{li2019nattack}                      & ICML 2019                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
Bandit \cite{ilyas2019prior}                       & ICLR 2019                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
ZO-signSGD \cite{liu2018signsgd}                   & ICLR 2019                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
SignHunter \cite{al2019sign}                       & ICLR 2019                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
Dong \etal \cite{dong2019efficient}                & CVPR 2019                 &     &     &     &     &     &     &     & \Circle              &                       \\
DI$^2$-FGSM \cite{DI-2019}                         & CVPR 2019                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
GeoDA \cite{rahmati2020geoda}                      & CVPR 2020                 &     &     &     &     &     &     &     & \Circle              &                       \\
QEBA  \cite{li2020qeba}                            & CVPR 2020                 &     &     &     &     &     &     &     & \Circle              &                       \\
TREMBA \cite{huang2020black}                       & ICLR 2020                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
Meta Attack \cite{du2020query}                     & ICLR 2020                 &     &     &     &     &     &     &     & \Circle              & \Circle                   \\
FDA \cite{FDA-2020}                                & ICLR 2020                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
SGM \cite{Wu2020Skip}                              & ICLR 2020                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
AdvFlow \cite{advflow}                             & NeurIPS 2020              &     &     &     &     &     &     &     & \CIRCLE              & \Circle                   \\
LinBP \cite{LinBP-2020}                            & NeurIPS 2020              &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
LeBA \cite{yang2020learning}                       & NeurIPS 2020              &     &     &     &     &     &     &     & \CIRCLE              &                       \\
Inkawhich \etal  \cite{inkawhich2020perturbing}    & NeurIPS 2020              &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
Suya \etal \cite{suya2020hybrid}                   & USENIX Security 2020      &     &     &     &     &     &     &     & \CIRCLE              &                       \\
Square attack \cite{ACFH2020square}                & ECCV 2020                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
SFA \cite{chen2020boosting}                        & ECCV 2020                 &     &     &     &     &     &     &     & \Circle              &                       \\
RayS \cite{chen2020rays}                           & ICDM 2020                 &     &     &     &     &     &     &     & \Circle              &                       \\
HopSkipJumpAttack \cite{chen2020hopskipjumpattack} & AAAI 2021                 &     &     &     &     &     &     &     & \Circle              &                       \\
EMI-FGSM \cite{wang2021boosting}                   & BMVC 2021                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
PI-FSGM \cite{wang2021boosting}                    & BMCV 2021                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
IR \cite{wang2021unified}                          & ICLR 2021                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
PRFA \cite{liang2021parallel}                      & ICCV 2021                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
MGAA \cite{metagradient2021}                       & ICCV 2021                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
Naseer \etal \cite{naseer2021generating}           & ICCV 2021                 &     &     &     &     &     &     &     & \Circle              & \Circle                   \\
Simulator attack \cite{ma2021simulating}           & CVPR 2021                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
VMI-FGSM \cite{Wang_2021_CVPR}                     & CVPR 2021                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
MSA \cite{yatsura2021meta}                         & NeurIPS 2021              &     &     &     &     &     &     &     & \CIRCLE              &                       \\
P-RGF \cite{dong2021query}                         & IEEE TPAMI 2021           &     &     &     &     &     &     &     & \CIRCLE              &                       \\
CG-Attack \cite{Feng2020CGATTACKMT}                & CVPR 2022                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
SVRE-MI-FGSM \cite{Xiong_2022_CVPR}                & CVPR 2022                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
CISA \cite{shi2022query}                           & IEEE TPAMI 2022           &     &     &     &     &     &     &     & \Circle              &                       \\
MCG \cite{my-pami2022-black-box}                   & IEEE TPAMI 2022           &     &     &     &     &     &     &     & \CIRCLE              & \Circle                   \\ \hline
\end{tabular}%
}
\end{table*}

==> tables/adversarial_papers_split.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage{longtable}
% Note: It may be necessary to compile the document several times to get a multi-page table to line up properly
\clearpage
\onecolumn
\begin{longtable}
{
m{0.07\textwidth}
m{0.06\textwidth}
|
m{0.065\textwidth}<{\centering}
m{0.08\textwidth}<{\centering}
m{0.07\textwidth}<{\centering}
m{0.07\textwidth}<{\centering}
m{0.05\textwidth}<{\centering}
m{0.075\textwidth}<{\centering}
m{0.07\textwidth}<{\centering}
|
m{0.07\textwidth}<{\centering}
m{0.07\textwidth}<{\centering}
}
\caption{Categorization of existing existing inference-time adversarial attack methods. For each categorization criterion ``A/B'', \Circle ~ denotes the former ``A'', \CIRCLE ~ denotes the latter ``B''.}
\label{tab:adversarial papers}\\
\hline
&& \multicolumn{7}{c|}{White-box attack}   & Black-box attack & Transfer-based attack \\

%

Method &
  Venue &
  \cellcolor[HTML]{FFF2CC}Digtial/ Physical &
  \cellcolor[HTML]{FFF2CC}Optimization / Learning-based &
  \cellcolor[HTML]{FFF2CC}Sample-agnostic/ specific &
  \cellcolor[HTML]{FFF2CC}Additive/ Non-additive &
  \cellcolor[HTML]{FFF2CC}Dense/ Sparse &
  \cellcolor[HTML]{D5E8D4}Untargeted/ Targeted &
  \cellcolor[HTML]{D5E8D4}Factorized/ Structured &
  \cellcolor[HTML]{E1D5E7}Decison/ Score-based &
  \cellcolor[HTML]{E1D5E7}Example/ Model-level \\ \hline
\endhead
Sharif \etal \cite{sharif2016accessorize}          & CCS 2016                  & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Kurakin \etal \cite{kurakin2018adversarial}        & ICLR 2017                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
UAP  \cite{moosavi2017universal}                   & CVPR 2017                 & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle &                  &                       \\
JSMA \cite{papernot2016limitations}                & EuroS\&P 2016             & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
Mopuri \etal \cite{mopuri2017fast}                 & BMVA 2017                 & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Carlini \etal \cite{carlini2017towards}            & IEEE S\&P 2017            & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
LocSearchAdv \cite{NarodytskaK16}                  & CVPR 2017                 & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
GD-UAP \cite{gd-uap-tpami-2018}                    & IEEE TPAMI 2018           & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Carlini \etal \cite{carlini2018audio}              & IEEE SPW 2018             & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \CIRCLE &                  &                       \\
ShapeShifter \cite{chen2018shapeshifter}           & ECML-PKDD 2018            & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
RP2 \cite{eykholt2018robust}                       & CVPR 2018                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Xu \etal \cite{xu2018fooling}                      & CVPR 2018                 & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \CIRCLE &                  &                       \\
Manifool \cite{kanbak2018geometric}                & CVPR 2018                 & \Circle & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle &                  &                       \\
Shi \etal \cite{shi2018learning}                   & COLING 2018               & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \CIRCLE &                  &                       \\
AC-GAN \cite{song2018constructing}                 & NeurIPS 2018              & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
advGAN \cite{xiao2018generating}                   & IJCAI 2018                & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
stAdv \cite{xiao2018spatially}                     & ICLR 2018                 & \Circle & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle &                  &                       \\
Athalye \cite{athalye2018synthesizing}             & ICML 2018                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
LaVAN \cite{karmon2018lavan}                       & ICML 2018                 & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
CGAN-Adv \cite{yu2018generating}                   & ICPR 2018                 & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Zhao \etal \cite{zhao2018admm}                     & MM 2018                   & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
Chen \etal \cite{chen2018attacking}                & ACL 2018                  & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \CIRCLE &                  &                       \\
Jan \etal \cite{jan2019connecting}                 & AAAI 2019                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Wei \etal \cite{WeiZYS19}                          & AAAI 2019                 & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
PS-GAN \cite{liu2019perceptual}                    & AAAI 2019                 & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
ERCG \cite{zhao2019seeing}                         & CCS 2019                  & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Qin \etal \cite{qin2019imperceptible}              & ICML 2019                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Engstrom \etal \cite{engstrom2019exploring}        & ICML 2019                 & \Circle & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle &                  &                       \\
Wong \etal \cite{wong2019wasserstein}              & ICML 2019                 & \Circle & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle &                  &                       \\
ReColorAdv \cite{laidlaw2019functional}            & NeurIPS 2019              & \Circle & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle &                  &                       \\
AT-GAN \cite{wang2019gan}                          & arXiv 2019                & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Yakura \etal \cite{yakura2018robust}               & IJCAI 2019                & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
AdvFaces  \cite{deb2019advfaces}                   & IJCB 2019                 & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
AGNs \cite{sharif2019general}                      & TOPS 2019                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
SparseFool \cite{ModasMF19}                        & CVPR 2019                 & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
Xu \etal \cite{xu2019exact}                        & CVPR 2019                 & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \CIRCLE &                  &                       \\
AdvPattern \cite{wang2019advpattern}               & ICCV 2019                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
CornerSearch \cite{croce2019sparse}                & ICCV 2019                 & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
PD-UA \cite{liu2019universal}                      & ICCV 2019                 & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Schott \etal \cite{SchottRBB19}                    & ICLR 2019                 & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
Xu \etal \cite{xu2018structured}                   & ICLR 2019                 & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
Su \etal \cite{su2019one}                          & IEEE TEC 2019             & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
CD-UAP \cite{cd-uap-aaai-2020}                     & AAAI 2020                 & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Xu \etal \cite{tshirt}                             & ECCV 2020                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Wu \etal \cite{wu2020making}                       & ECCV 2020                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
SAPF \cite{my-eccv-sparse}                         & ECCV 2020                 & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
UPC  \cite{huang2020universal}                     & CVPR 2020                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
AdvCam \cite{duan2020adversarial}                  & CVPR 2020                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
LG-GAN \cite{zhou2020lg}                           & CVPR 2020                 & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Xu \etal \cite{xu2020machines}                     & CVPR 2020                 & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \CIRCLE &                  &                       \\
PhysGAN \cite{kong2020physgan}                     & CVPR 2020                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Li \etal \cite{li2020towards}                      & CVPR 2020                 & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \CIRCLE & \Circle &                  &                       \\
GreedyFool \cite{LiuZGAL20}                        & NeurIPS 2020              & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle &                  &                       \\
Xu \etal \cite{xu2020learning}                     & MM 2020                   & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \CIRCLE &                  &                       \\
MAG-GAN \cite{chen2020mag}                         & Information Sciences 2020 & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
GUAP \cite{zhang2020generalizing}                  & ICDM 2020                 & \Circle & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle &                  &                       \\
Wong \etal \cite{wong2020learning}                 & ICLR 2021                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
AdvHat \cite{komkov2021advhat}                     & ICPR 2021                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Sayles \etal \cite{sayles2021invisible}            & CVPR 2021                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
TTP \cite{naseer2021generating}                    & ICCV 2021                 & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \CIRCLE & \Circle &                  &                       \\
CMML  \cite{feng2021meta}                          & ICCV 2021                 & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
Zhao \etal \cite{zhao2021success}                  & NeurIPS 2021              & \Circle & \Circle & \CIRCLE & \Circle & \Circle & \CIRCLE & \Circle &                  &                       \\
SLAP \cite{lovisotto2021slap}                      & USENIX Security 2021      & \CIRCLE & \Circle & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\
AP-GAN \cite{zhao2020ap}                           & Geoinformatica 2022       & \Circle & \CIRCLE & \CIRCLE & \Circle & \Circle & \Circle & \Circle &                  &                       \\ \hline\hline
Brendel \etal \cite{brendel2018decision}           & ICLR 2018                 &     &     &     &     &     &     &     & \Circle              &                       \\
Ilyas \etal \cite{ilyas2018black}                  & ICML 2018                 &     &     &     &     &     &     &     & \Circle              &                       \\
NES \cite{ilyas2018black}                          & ICML 2018                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
GAP \cite{gap-2018}                                & CVPR 2018                 &     &     &     &     &     &     &     &                  & \Circle                   \\
MI-FGSM \cite{dong2018boosting}                    & CVPR 2018                 &     &     &     &     &     &     &     &                  & \CIRCLE                   \\
OPT \cite{cheng2019query}                          & ICLR 2019                 &     &     &     &     &     &     &     & \Circle              &                       \\
Sign-OPT \cite{cheng2019improving}                 & NeurIPS 2019              &     &     &     &     &     &     &     & \Circle              &                       \\
Subspace attack \cite{guo2019subspace}             & NeurIPS 2019              &     &     &     &     &     &     &     & \CIRCLE              &                       \\
Naseer \etal \cite{naseer2019cross}                & NeurIPS 2019              &     &     &     &     &     &     &     & \Circle              & \Circle                   \\
qFool \cite{liu2019geometry}                       & ICCV 2019                 &     &     &     &     &     &     &     & \Circle              &                       \\
ILAP \cite{huang2019enhancing}                     & ICCV 2019                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
SimBA \cite{guo2019simple}                         & ICML 2019                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
ECO \cite{moon2019parsimonious}                    & ICML 2019                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
NAttack  \cite{li2019nattack}                      & ICML 2019                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
Bandit \cite{ilyas2019prior}                       & ICLR 2019                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
ZO-signSGD \cite{liu2018signsgd}                   & ICLR 2019                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
SignHunter \cite{al2019sign}                       & ICLR 2019                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
Dong \etal \cite{dong2019efficient}                & CVPR 2019                 &     &     &     &     &     &     &     & \Circle              &                       \\
DI$^2$-FGSM \cite{DI-2019}                         & CVPR 2019                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
GeoDA \cite{rahmati2020geoda}                      & CVPR 2020                 &     &     &     &     &     &     &     & \Circle              &                       \\
QEBA  \cite{li2020qeba}                            & CVPR 2020                 &     &     &     &     &     &     &     & \Circle              &                       \\
TREMBA \cite{huang2020black}                       & ICLR 2020                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
Meta Attack \cite{du2020query}                     & ICLR 2020                 &     &     &     &     &     &     &     & \Circle              & \Circle                   \\
FDA \cite{FDA-2020}                                & ICLR 2020                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
SGM \cite{Wu2020Skip}                              & ICLR 2020                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
AdvFlow \cite{advflow}                             & NeurIPS 2020              &     &     &     &     &     &     &     & \CIRCLE              & \Circle                   \\
LinBP \cite{LinBP-2020}                            & NeurIPS 2020              &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
LeBA \cite{yang2020learning}                       & NeurIPS 2020              &     &     &     &     &     &     &     & \CIRCLE              &                       \\
Inkawhich \etal  \cite{inkawhich2020perturbing}    & NeurIPS 2020              &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
Suya \etal \cite{suya2020hybrid}                   & USENIX Security 2020      &     &     &     &     &     &     &     & \CIRCLE              &                       \\
Square attack \cite{ACFH2020square}                & ECCV 2020                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
SFA \cite{chen2020boosting}                        & ECCV 2020                 &     &     &     &     &     &     &     & \Circle              &                       \\
RayS \cite{chen2020rays}                           & ICDM 2020                 &     &     &     &     &     &     &     & \Circle              &                       \\
Hop Skip Jump Attack \cite{chen2020hopskipjumpattack} & AAAI 2021                 &     &     &     &     &     &     &     & \Circle              &                       \\
EMI-FGSM \cite{wang2021boosting}                   & BMVC 2021                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
PI-FSGM \cite{wang2021boosting}                    & BMCV 2021                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
IR \cite{wang2021unified}                          & ICLR 2021                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
PRFA \cite{liang2021parallel}                      & ICCV 2021                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
MGAA \cite{metagradient2021}                       & ICCV 2021                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
Naseer \etal \cite{naseer2021generating}           & ICCV 2021                 &     &     &     &     &     &     &     & \Circle              & \Circle                   \\
Simulator attack \cite{ma2021simulating}           & CVPR 2021                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
VMI-FGSM \cite{Wang_2021_CVPR}                     & CVPR 2021                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
MSA \cite{yatsura2021meta}                         & NeurIPS 2021              &     &     &     &     &     &     &     & \CIRCLE              &                       \\
P-RGF \cite{dong2021query}                         & IEEE TPAMI 2021           &     &     &     &     &     &     &     & \CIRCLE              &                       \\
CG-Attack \cite{Feng2020CGATTACKMT}                & CVPR 2022                 &     &     &     &     &     &     &     & \CIRCLE              &                       \\
SVRE-MI-FGSM \cite{Xiong_2022_CVPR}                & CVPR 2022                 &     &     &     &     &     &     &     & \Circle              & \CIRCLE                   \\
CISA \cite{shi2022query}                           & IEEE TPAMI 2022           &     &     &     &     &     &     &     & \Circle              &                       \\
MCG \cite{my-pami2022-black-box}                   & IEEE TPAMI 2022           &     &     &     &     &     &     &     & \CIRCLE              & \Circle                   \\ \hline
\end{longtable}
\twocolumn

==> tables/backdoor_category.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[t]
\centering
\renewcommand\arraystretch{1.4}
\newcolumntype{P}[1]{>{\raggedright\arraybackslash}p{#1}}
\caption{Summary of different categorizations of backdoor attacks. Each row indicates one perspective to categorize existing attacks.}
\label{tab: backdoor attacks}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l m{.35\textwidth}  l m{.35\textwidth}}
\hline
\multicolumn{4}{c}{General formulation of backdoor attack}                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\
\multicolumn{4}{c}{$\arg\min_{\x_{\varepsilon} \in \mathcal{C}_{\x}, \w_{\varepsilon} \in \mathcal{C}_{\w}} ~ \frac{1}{N_{0}}\sum_{i=1}^{N_{0}} \lambda_3 \cL_3(f_{\w_{\varepsilon}}(\x_0), y_0) + \frac{1}{N_{\varepsilon}} \sum_{i=1}^{N_{\varepsilon}} \big[ \D_1(\x_0, \x_{\varepsilon}) + \lambda_5 \cL_5(f_{\w_{\varepsilon}}(\x_{\varepsilon}), y_{\varepsilon}) + \lambda_{r_2} \mathcal{R}_2(f_{\w_{\varepsilon}}(\x_0), f_{\w_{\varepsilon}}(\x_{\varepsilon})) \big]$} \\ \hline\hline
\multicolumn{4}{c}{Data-poisoning based backdoor attacks}                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
\cellcolor[HTML]{FFF2CC}$\scriptscriptstyle\bigDiamond$ Visible trigger                   & $\x_{\varepsilon} - \x_0$ is visible to human perception, but will not interfere human's prediction                                                  & \cellcolor[HTML]{FFF2CC}$\scriptscriptstyle\bigLozenge$ Invisible trigger                   & $\x_{\varepsilon} - \x_0$ is too small to be perceived by human perception                                                                                                    \\
\cellcolor[HTML]{FFF2CC}$\scriptscriptstyle\bigDiamond$ Non-semantic trigger              & There is no semantic connection between $\x_{\varepsilon} - \x_0$ and $\x_0$                                                                         & \cellcolor[HTML]{FFF2CC}$\scriptscriptstyle\bigLozenge$ Semantic trigger                    & There is semantic connection between $\x_{\varepsilon} - \x_0$ and $\x_0$. For example, $\x_{\varepsilon} - \x_0$ is a semantic part of $\x_0$, \textbackslash{}eg, a red hat \\
\cellcolor[HTML]{FFF2CC}$\scriptscriptstyle\bigDiamond$ Manually designed trigger         & The trigger $\bm{\varepsilon}$ is not learned during the training process. In other words, $\x_{\varepsilon}$ is constant in the above formulation.  & \cellcolor[HTML]{FFF2CC}$\scriptscriptstyle\bigLozenge$ Learnable trigger                   & The trigger $\bm{\varepsilon}$ is learned along with the model parameter $\w_{\varepsilon}$                                                                                   \\ \hline
\cellcolor[HTML]{FFE6CC}$\scriptscriptstyle\bigDiamond$ Additive trigger                  & $\x_{\varepsilon} =  \alpha \x_0 + (1-\alpha) \bm{\varepsilon}$                                                                                      & \cellcolor[HTML]{FFE6CC}$\scriptscriptstyle\bigLozenge$ Non-additive trigger                & $\x_{\varepsilon} =  g(\x_0, \bm{\varepsilon})$, with $g(\cdot)$ being a non-additive transformation function                                                                 \\
\cellcolor[HTML]{FFE6CC}$\scriptscriptstyle\bigDiamond$ Static trigger                    & $\x_{\varepsilon} - \x_0$ keeps static in each adversarial input $\x_{\varepsilon}$, such as fixed location, fixed shape and fixed appearance        & \cellcolor[HTML]{FFE6CC}$\scriptscriptstyle\bigLozenge$ Dynamic trigger                     & $\x_{\varepsilon} - \x_0$ may vary randomly or following some rules in different adversarial inputs $\x_{\varepsilon}$                                                        \\
\cellcolor[HTML]{FFE6CC}$\scriptscriptstyle\bigDiamond$ Sample-agnostic trigger           & $\x_{\varepsilon} - \x_0$ is independent with any specific $\x_0$                                                                                    & \cellcolor[HTML]{FFE6CC}$\scriptscriptstyle\bigLozenge$ Sample-specific trigger             & $\x_{\varepsilon} - \x_0$ depends on $\x_0$ and is different for each $\x_0$                                                                                                  \\ \hline
\cellcolor[HTML]{D5E8D4}$\scriptscriptstyle\bigDiamond$ Label-inconsistent attack         & The poisoned sample $\x_{\varepsilon}$ looks inconsistent with its label $y_{\varepsilon}$, from human's perspective                                 & \cellcolor[HTML]{D5E8D4}$\scriptscriptstyle\bigLozenge$ Label-consistent attack             & The poisoned sample $\x_{\varepsilon}$ looks consistent with its label $y_{\varepsilon}$, from human's perspective                                                            \\
\cellcolor[HTML]{D5E8D4}$\scriptscriptstyle\bigDiamond$ Single-target class               & $y_{\varepsilon}$ is a single class                                                                                                                  & \cellcolor[HTML]{D5E8D4}$\scriptscriptstyle\bigLozenge$ Multi-target classes                & $y_{\varepsilon}$ could be a set of multiple target classes, often corresponding to multiple triggers                                                                         \\ \hline\hline
\multicolumn{4}{c}{Training-controllable based backdoor attack}                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ \hline
\cellcolor[HTML]{E1D5E7}$\scriptscriptstyle\bigDiamond$ One-stage training                & $\x_{\varepsilon}$ and $\w_{\varepsilon}$ are learned simultaneously                                                                                 & \cellcolor[HTML]{E1D5E7}$\scriptscriptstyle\bigLozenge$ Two-stage training                  & $\x_{\varepsilon}$ and $\w_{\varepsilon}$ are learned in two separated stages                                                                                                 \\
\cellcolor[HTML]{E1D5E7}$\scriptscriptstyle\bigDiamond$ Full access of training data      & The attacker can access and manipulate all training data                                                                                             & \cellcolor[HTML]{E1D5E7}$\scriptscriptstyle\bigLozenge$ Partial access of training data     & The attacker can access and manipulate only a partial set of training data                                                                                                    \\
\cellcolor[HTML]{E1D5E7}$\scriptscriptstyle\bigDiamond$ Full control of training process  & The attacker can control the whole training process                                                                                                  & \cellcolor[HTML]{E1D5E7}$\scriptscriptstyle\bigLozenge$ Partial control of training process & The attacker can only control a part of the whole training process                                                                                                            \\ \hline
\end{tabular}%
}
\end{table*}

==> tables/backdoor_papers.tex <==




% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[ht]
\caption{Categorization of existing training-time adversarial attack (\ie, backdoor attack) methods. For each categorization criterion ``A/B'', \Circle ~denotes the former ``A'', \CIRCLE ~ denotes the latter ``B'' and \RIGHTcircle ~ represents both. For criterion ``A/B/C/D'', \Circle , \CIRCLE, \LEFTCIRCLE, \RIGHTCIRCLE denote ``A'', ``B'', ``C'' , ``D'' respectively. For the methods of partially controlling the training data and process, we omit trigger since there is no distinguishable trigger listed in the table.}
\label{tab:backdoor papers}
\renewcommand\arraystretch{1.4}
\resizebox{\textwidth}{!}{%
\begin{tabular}
{
m{0.09\textwidth}
m{0.09\textwidth} |
m{0.06\textwidth}<{\centering}
m{0.07\textwidth}<{\centering}
m{0.07\textwidth}<{\centering}
m{0.07\textwidth}<{\centering}
m{0.07\textwidth}<{\centering}
m{0.07\textwidth}<{\centering}
m{0.07\textwidth}<{\centering}
m{0.07\textwidth}<{\centering}
m{0.08\textwidth}<{\centering} |
m{0.07\textwidth}<{\centering}
m{0.09\textwidth}<{\centering}
m{0.09\textwidth}<{\centering}
m{0.09\textwidth}<{\centering}
}
\hline
 &
   &
  \multicolumn{9}{c|}{Data-poisoning based backdoor attack} &
  \multicolumn{4}{c}{Training-controllable based backdoor attack} \\
Method &
  Venue &
  \cellcolor[HTML]{FFF2CC}Visible / Invisible &
  \cellcolor[HTML]{FFF2CC}Non-semantic / Semantic &
  \cellcolor[HTML]{FFF2CC}Manually designed / Leanable &
  \cellcolor[HTML]{FFF2CC}Digital / Physical &
  \cellcolor[HTML]{FFE6CC}Additive / Non-additive &
  \cellcolor[HTML]{FFE6CC}Static / Dynamic &
  \cellcolor[HTML]{FFE6CC}Sample-agnostic / specific &
  \cellcolor[HTML]{D5E8D4}Label-inconsistent / consistent &
  \cellcolor[HTML]{D5E8D4}Single / Multi-target &
  \cellcolor[HTML]{E1D5E7}One / Two-stage &
  \cellcolor[HTML]{E1D5E7}Full / Partial access of training data &
  \cellcolor[HTML]{E1D5E7}Full / Partial control of training process &
  \cellcolor[HTML]{E1D5E7}Controlling training loss / algorithm / indices / order \\ \hline
BadNets \cite{gu2019badnets} &
  IEEE Access 2019 &
  \Circle &
  \Circle &
  \Circle &
  \RIGHTcircle &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \RIGHTcircle &
   &
   &
   &
   \\
Blended \cite{chen2017targeted} &
  arXiv 2017 &
  \CIRCLE &
  \Circle &
  \Circle &
  \RIGHTcircle &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
   &
   &
   &
   \\
Shafahi \etal \cite{shafahi2018poison} &
  NeurIPS 2018 &
  \CIRCLE &
  \Circle &
  \CIRCLE &
  \Circle &
  \CIRCLE &
  \CIRCLE &
  \CIRCLE &
  \CIRCLE &
  \Circle &
   &
   &
   &
   \\
SIG \cite{barni2019new} &
  ICIP 2019 &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
   &
   &
   &
   \\
LC \cite{turner2019labelconsistent} &
  arXiv 2019 &
  \CIRCLE &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \CIRCLE &
  \CIRCLE &
  \CIRCLE &
  \Circle &
   &
   &
   &
   \\
Saha \etal \cite{saha2020hidden} &
  AAAI2020 &
  \CIRCLE &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \CIRCLE &
  \CIRCLE &
  \CIRCLE &
  \Circle &
   &
   &
   &
   \\
Static \cite{zhong2020backdoor} &
  CODASPY 2020 &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
   &
   &
   &
   \\
Adaptive \cite{zhong2020backdoor} &
  CODASPY 2020 &
  \CIRCLE &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
   &
   &
   &
   \\
Zhao \etal \cite{zhao2020clean} &
  CVPR 2020 &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
   &
   &
   &
   \\
Refool \cite{liu2020reflection} &
  ECCV 2020 &
  \CIRCLE &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
  \CIRCLE &
  \Circle &
   &
   &
   &
   \\
Li \etal \cite{li2020light} &
  arXiv 2020 &
  \CIRCLE &
  \Circle &
  \CIRCLE &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
   &
   &
   &
   \\
DeHiB \cite{yan2021dehib} &
  AAAI 2021 &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \CIRCLE &
  \CIRCLE &
  \CIRCLE &
  \Circle &
   &
   &
   &
   \\
Wenger \etal \cite{wenger2021backdoor} &
  CVPR 2021 &
  \Circle &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
   &
   &
   &
   \\
Li \etal \cite{li2021hidden} &
  CCS 2021 &
  \CIRCLE &
  \CIRCLE &
  \Circle &
  \Circle &
  \CIRCLE &
  \CIRCLE &
  \CIRCLE &
  \Circle &
  \Circle &
   &
   &
   &
   \\
Steganography \cite{li2020invisible} &
  IEEE TDSC 2021 &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \CIRCLE &
  \CIRCLE &
  \Circle &
  \Circle &
   &
   &
   &
   \\
Regularization \cite{li2020invisible} &
  IEEE TDSC 2021 &
  \CIRCLE &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
   &
   &
   &
   \\
Invisible Poison \cite{ninginvisible} &
  INFOCOM 2021 &
  \CIRCLE &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
   &
   &
   &
   \\
ROBNET \cite{gong2021defense} &
  IEEE JSAC 2021 &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \RIGHTcircle &
   &
   &
   &
   \\
AdvDoor \cite{zhang2021advdoor} &
  ISSTA 2021 &
  \CIRCLE &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
   &
   &
   &
   \\
SSBA  \cite{li2021invisible} &
  ICCV 2021 &
  \CIRCLE &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \CIRCLE &
  \CIRCLE &
  \Circle &
  \Circle &
   &
   &
   &
   \\
Random Backdoor \cite{salem2022dynamic} &
  Euro S\&P 2022 &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \RIGHTcircle &
   &
   &
   &
   \\
Sleeper Agent \cite{souri2021sleeper} &
  NeurIPS 2022 &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
  \CIRCLE &
  \Circle &
   &
   &
   &
   \\
PTB \cite{xue2022ptb} &
  C \& S 2022 &
  \Circle &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
   &
   &
   &
   \\
FaceHack \cite{sarkar2020facehack} &
  IEEE TBBIS 2022 &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
  \CIRCLE &
  \CIRCLE &
  \CIRCLE &
  \Circle &
  \Circle &
   &
   &
   &
   \\
Han \etal \cite{han2022physical} &
  MM 2022 &
  \Circle &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
  \RIGHTcircle &
  \Circle &
   &
   &
   &
   \\
IRBA \cite{gao2022imperceptible} &
  arXiv 2022 &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
  \CIRCLE &
  \CIRCLE &
  \CIRCLE &
  \Circle &
  \Circle &
   &
   &
   &
   \\ \hline \hline
Bhagoji \etal \cite{bhagoji2019analyzing} &
  ICML 2019 &
   &
   &
   &
  \Circle &
   &
   &
   &
   &
   &
   &
  \CIRCLE &
   &
  \CIRCLE \\
Bagdasaryan \etal \cite{bagdasaryan2020backdoor} &
  AISTATS 2020 &
   &
   &
   &
  \Circle &
   &
   &
  \textbf{} &
   &
   &
   &
  \CIRCLE &
   &
  \CIRCLE \\
Wang \etal \cite{wang2020attack-fed} &
  NeurIPS 2020 &
   &
   &
   &
  \Circle &
   &
   &
   &
   &
   &
   &
  \CIRCLE &
   &
  \CIRCLE \\
Fung \etal \cite{fung2020limitations} &
  RAID 2020 &
   &
   &
   &
  \Circle &
   &
   &
   &
   &
   &
   &
  \CIRCLE &
   &
  \CIRCLE \\
Chen \etal \cite{chen2020backdoor} &
  arXiv 2020 &
   &
   &
   &
  \Circle &
   &
   &
   &
   &
   &
   &
  \CIRCLE &
   &
  \CIRCLE \\
Liu \etal \cite{liu2020backdoor} &
  arXiv 2020 &
   &
   &
   &
  \Circle &
   &
   &
   &
   &
   &
   &
  \CIRCLE &
   &
  \CIRCLE \\
Composite Attack \cite{lin2020composite} &
  CCS 2020 &
  \Circle &
  \CIRCLE &
  \Circle &
  \RIGHTcircle &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
   &
   &
  \CIRCLE \\
DBA \cite{xie2019dba} &
  ICLR 2020 &
   &
   &
   &
  \Circle &
   &
   &
   &
   &
   &
   &
  \CIRCLE &
   &
  \CIRCLE \\
Nguyen \etal \cite{nguyen2020input} &
  NeurIPS 2020 &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \CIRCLE &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
   &
   &
  \CIRCLE \\
DFST \cite{cheng2020deep} &
  AAAI 2021 &
  \CIRCLE &
  \Circle &
  \CIRCLE &
  \Circle &
  \CIRCLE &
  \CIRCLE &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
   &
   &
  \CIRCLE \\
WaNet \cite{nguyen2021wanet} &
  ICLR 2021 &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
  \CIRCLE &
  \CIRCLE &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
   &
   &
  \CIRCLE \\
WB \cite{doan2021backdoor} &
  NeurIPS 2021 &
  \CIRCLE &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \CIRCLE &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
   &
   &
  \Circle \\
BOB \cite{ordering-attack-nips-2021} &
  NeurIPS 2021 &
   &
   &
   &
  \Circle &
   &
   &
   &
   &
   &
   &
   &
   &
  \RIGHTCIRCLE \\
LIRA \cite{doan2021lira} &
  ICCV 2021 &
  \CIRCLE &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
  \Circle &
   &
   &
  \CIRCLE \\
LWP \cite{lwp2021backdoor} &
  EMNLP 2021 &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
  \CIRCLE &
  \CIRCLE \\
Shen \etal \cite{shen2021backdoor} &
  CCS 2021 &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
  \CIRCLE &
  \CIRCLE \\
BaN \cite{salem2022dynamic} &
  Euro S\&P 2022 &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \CIRCLE &
  \CIRCLE &
  \Circle &
  \RIGHTcircle &
  \Circle &
   &
   &
  \CIRCLE \\
c-BaN \cite{salem2022dynamic} &
  Euro S\&P 2022 &
  \Circle &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \CIRCLE &
  \CIRCLE &
  \Circle &
  \RIGHTcircle &
  \Circle &
   &
   &
  \CIRCLE \\
Zhong \etal \cite{zhong2022imperceptible} &
  IJCAI 2022 &
  \CIRCLE &
  \Circle &
  \CIRCLE &
  \Circle &
  \Circle &
  \CIRCLE &
  \CIRCLE &
  \Circle &
  \Circle &
  \Circle &
   &
   &
  \CIRCLE \\
FUS \cite{data-efficient-backdoor-2022} &
  IJCAI 2022 &
   &
   &
   &
  \Circle &
   &
   &
   &
   &
   &
   &
   &
   &
  \LEFTCIRCLE \\
PPT \cite{duppt} &
  IJCAI 2022 &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   &
  \CIRCLE &
  \CIRCLE \\
Wen \etal \cite{wen2022thinking} &
  arXiv 2022 &
   &
   &
   &
  \Circle &
   &
   &
   &
   &
   &
   &
  \CIRCLE &
   &
  \CIRCLE \\
BPPATTACK \cite{wang2022bppattack} &
  CVPR 2022 &
   &
   &
   &
  \Circle &
   &
   &
   &
   &
   &
   &
   &
   &
  \Circle \\ \hline
\end{tabular}%
}
\end{table*}
